Fusion-in-T5: Unifying Document Ranking Signals for Improved Information Retrieval

Common document ranking pipelines in search systems are cascade systems that involve multiple ranking layers to integrate different information step-by-step. In this paper, we propose a novel re-ranker Fusion-in-T5 (FiT5), which integrates text matching information, ranking features, and global document information into one single unified model via templated-based input and global attention. Experiments on passage ranking benchmarks MS MARCO and TREC DL show that FiT5, as one single model, significantly improves ranking performance over complex cascade pipelines. Analysis finds that through attention fusion, FiT5 jointly utilizes various forms of ranking information via gradually attending to related documents and ranking features, and improves the detection of subtle nuances. Our code is open-sourced at https://github.com/OpenMatch/FiT5.

==> limitations.tex <==
\section*{Limitations}

FiT5 requires the construction of a fully-connected global attention graph for each query. Currently, our implementation necessitates that all candidate documents for a given query reside on the same GPU. In our experiments, we re-rank the top 100 documents, which can be accomplished efficiently using a single A100 40G GPU. However, in certain situations, users may desire to re-rank a larger number of documents, such as the top 1000, in order to achieve better results. In such cases, running FiT5 with a fully connected global attention graph on all documents becomes infeasible. To address this challenge, one approach is to train on smaller graphs, for instance, the top 100 documents, and during inference, divide all candidate documents (e.g., top 1000 documents) into smaller shards (e.g., 100 document shards). Inference can then be performed on these shards, followed by the merging of results. Another solution involves modifying our code to support graph parallelization, enabling the distribution of global attention calculations across multiple GPU devices.

To demonstrate the efficacy of attention fusion, we currently utilize only the most fundamental ranking feature—the retrieval score—in our input. However, it is possible to incorporate additional ranking features, which are expected to yield more substantial empirical improvements.
